The COMPASS Experiment at CERN

The COMPASS experiment makes use of the CERN SPS high-intensitymuon and hadron beams for the investigation of the nucleon spin structure and the spectroscopy of hadrons. One or more outgoing particles are detected in coincidence with the incoming muon or hadron. A large polarized target inside a superconducting solenoid is used for the measurements with the muon beam. Outgoing particles are detected by a two-stage, large angle and large momentum range spectrometer. The setup is built using several types of tracking detectors, according to the expected incident rate, required space resolution and the solid angle to be covered. Particle identification is achieved using a RICH counter and both hadron and electromagnetic calorimeters. The setup has been successfully operated from 2002 onwards using a muon beam. Data with a hadron beam were also collected in 2004. This article describes the main features and performances of the spectrometer in 2004; a short summary of the 2006 upgrade is also given.

==> compass_spec_dcs.tex <==
\section{Detector Control System}
\label{sec:dcs}
The Detector Control System (DCS) aims at guaranteeing a reliable and 
stable operation of the COMPASS detector, from one single remote point. 
All the control and monitoring tasks are performed from a central room, 
avoiding losses of beam time to access equipments placed in the experimental 
area. The DCS architecture consists of the supervisory layer, offering 
monitoring and control capabilities, with a graphical user interface, alert 
handling, data trending, processing and archiving of historical values; 
the front-ends layer, comprising the specific software and hardware for 
controls and interfacing; and the devices layer, including all the hardware to 
control, as well as sensors for the monitored parameters. For the supervisory 
layer, a commercial SCADA, the package PVSS-II~\cite{PVSS:05}, is used. 
Non-standard equipments are integrated in the DCS by using specifically 
developed front-end software.

From the point of view of their operation, the COMPASS sub-detectors are 
independent from each other. There is no uniformity in the choices made by 
each responsible group for their sub-systems, and this variety of different 
equipments leads to a complex architecture at both the front-ends and the 
supervisory level of the DCS.

\subsection{The devices layer}

The devices to control are distributed along $50~\,m$ in the 
experimental area, and also spread at the end of the beam tunnel and in 
the electronics rooms. The requirements for slow control include: 
\begin{itemize}
\item control of crates and power supplies; 
\item monitoring of voltages and currents in crates and power supplies; 
\item control of high voltage channels; 
\item monitoring of temperatures, humidities, pressures and magnetic fields 
in specific points of the experimental hall, sub-detectors and magnets; 
\item monitoring of gas fluxes and mixtures in gaseous chambers. 
\end{itemize}
Standard commercial solutions for these control and monitoring tasks are 
adopted, whenever these are available and meet the performance and budgetary 
requirements of the experiment.
 
The high voltage systems use mainly CAEN modules, with the exception of two 
sub-detectors that use also ISEG modules. For CAEN high voltage power supplies,
 the proprietary fieldbus CAENET is used; and in the case of one crate of new 
type, offering for the first time this possibility, Ethernet is also used. 
5 CAENET buses connect a total of 22 crates in daisy chains ($\approx$ 
1200 high voltage channels). For the other power supplies, the connection to slow 
control is done using the industry standard CAN. Several CANbuses 
are used to connect ISEG high voltage crates ($\approx$ 340 channels), and 
WIENER fan-trays (for 15 VME 9U crates) to the slow control.

COMPASS uses extensively the multi-purpose I/O system ELMB (Embedded Local 
Monitor Board)~\cite{Hallgren:01} developed at CERN for the ATLAS experiment. 
The ELMB solution was selected by COMPASS since it provides multiplexed 
ADC readings for analog measurements, at low cost per channel. A total of 
28 ELMBs are used, providing 800 analog measurements.

The gas systems of several detectors are controlled by PLCs (Programmable 
Logic Controllers), that act on mass flowmeters to ensure constant and 
correct gas flows and mixtures. The relevant parameters to monitor are sent 
via serial connection to a front-end DCS computer, where an OPC server makes 
them available to the PVSS client. 

\subsection{The front-ends layer}

At the front-ends level, the CAN fieldbuses connect Windows computers, 
where commercial or custom OPC servers run. The choice of OPC servers 
is a natural one, since their use reduces significantly the development work 
for slow control of standard equipment, and technical support is usually 
offered. 

In the specific cases of equipments for which no commercial OPC server is 
available, or when this does not meet the performance requirements of the 
experiment, custom SLiC~\cite{Beharrel:05} servers are implemented, using OPC 
or DIM~\cite{Gaspar:01} communication protocols. For the CAEN high voltage 
systems, a SLiC DIM server was chosen, since no proprietary OPC server was 
available at the time. The SLiC server has several lists of items to survey, 
each with a tunable cycle speed. A fast cycle is used for the monitored 
voltages, currents and channel status, with speeds of $10 - 20\,ms$/channel. 
A slow cycle is also defined, for the readback of setting values. 

The control of one CAEN crate of new type is done using the CAEN OPC 
server. This OPC server presented many problems during the first months of 
use, that were only cured by new version releases of this software.

Another SLiC DIM server is used for the control of VME crate fan-trays. 
This choice was motivated by the unavailability at the time of a 
commercial OPC server. The ISEG high voltage systems of 2 sub-detectors 
are controlled by a SLiC OPC server. This server was developed at COMPASS, 
together with a framework for full integration. The ELMBs used for analog 
measurements connect via CANbus to an OPC server developed at CERN, based on 
the CANOpen protocol~\cite{ELMB:05}.

\subsection{The supervisory layer}

PVSS-II is a commercial product originally designed for industrial controls, 
and it lacks some functionalities needed in high energy physics experiments. To 
overcome this, a software tool, the JCOP-Framework~\cite{Myers:99}, was 
developed at CERN, including guidelines, tools and libraries that simplify the 
development work needed to integrate standard equipments in PVSS. This and an 
additional small COMPASS framework are used in the DCS. 

PVSS-II is device-oriented and its functioning is event-driven (as opposed 
to cyclic), thus avoiding unnecessary data traffic and offering good 
time performances. PVSS clients connect to the OPC and DIM servers, 
subscribing to lists of items. The DIM servers are distributed in Windows and 
Linux computers, in general placed close to the front-end electronics. The 
OPC servers and PVSS OPC clients run in several Windows computers. All these 
connect via TCP/IP to the main Linux DCS computer, where the PVSS core 
runs. Figure~\ref{figure:dcs} shows a schematic view of the DCS 
architecture.
\begin{figure*}[tbp]
  \begin{center}
    \includegraphics[width=\textwidth]{./figures/DCS}
  \end{center}
  \caption{The architecture of the Detector Control System}
  \label{figure:dcs}
\end{figure*}


\subsection{Performance issues}

During the data taking periods from 2002 to 2004, the DCS system 
has been extended and improved, becoming more robust and running stable. 
The reliability of the system is guaranteed by a regular backup policy of the 
whole DCS project; by the export of the historical data into external 
storage systems; and by connecting the main DCS computers to safety UPS units. 
The remaining problems that have been identified at the level of the 
software were solved with new release versions of the packages used. The 
recent PVSS-II version 3.0 lead to a new version of the JCOP-Framework, where 
a new architecture philosophy was applied, more adapted to high-energy physics 
needs. The 2005 SPS shutdown provided the opportunity to redesign the DCS 
system of COMPASS, making use of the new packages and structuring the project 
in a more coherent manner. 



==> dumm <==
This is pdfTeXk, Version 3.141592-1.40.3 (Web2C 7.5.6)
 %&-line parsing enabled.
entering extended mode
(./compass_spec.tex
LaTeX2e <2005/12/01>
Babel <v3.8h> and hyphenation patterns for english, usenglishmax, dumylang, noh
yphenation, arabic, basque, bulgarian, coptic, welsh, czech, slovak, german, ng
erman, danish, esperanto, spanish, catalan, galician, estonian, farsi, finnish,
 french, greek, monogreek, ancientgreek, croatian, hungarian, interlingua, ibyc
us, indonesian, icelandic, italian, latin, mongolian, dutch, norsk, polish, por
tuguese, pinyin, romanian, russian, slovenian, uppersorbian, serbian, swedish, 
turkish, ukenglish, ukrainian, loaded.
(./elsart3p.cls
Document Class: elsart3p 2006/05/01, 2.19: Elsevier
(./elsart.cls
Document Class: elsart 2006/05/01, 2.19: Elsevier
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/latex/base/latexsym.sty)
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/latex/base/ulasy.fd)))
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/latex/graphics/graphicx.sty
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/latex/graphics/keyval.sty)
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/latex/graphics/graphics.sty
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/latex/graphics/trig.sty)
(/afs/cern.ch/sw/XML/TL2007/texmf/tex/latex/config/graphics.cfg)
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/latex/pdftex-def/pdftex.def)))
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/latex/oberdiek/epstopdf.sty

Package epstopdf Warning: Shell escape feature is not enabled.

) (/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/generic/babel/babel.sty
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/generic/babel/english.ldf
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/generic/babel/babel.def)))
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/latex/amsfonts/amssymb.sty
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(./myunits.sty Document Style Option `myunits' Version 1.1 of 9 Aug 2000)
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/latex/carlisle/fix2col.sty)
(./compass_spec.aux (./compass_spec_tit.aux) (./compass_spec_int.aux)
(./compass_spec_lay.aux) (./compass_spec_bea.aux) (./compass_spec_tgt.aux)
(./compass_spec_trk.aux) (./compass_spec_pid.aux) (./compass_spec_trg.aux)
(./compass_spec_daq.aux) (./compass_spec_onl.aux) (./compass_spec_per.aux)
(./compass_spec_upg.aux) (./compass_spec_sum.aux) (./compass_spec_ack.aux))
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/context/base/supp-pdf.tex
[Loading MPS to PDF converter (version 2006.09.02).]
) (./compass_spec_tit.tex
Overfull \vbox (11.80556pt too high) detected at line 6

Overfull \vbox (9.0pt too high) detected at line 9

Overfull \vbox (8.19998pt too high) detected at line 11
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/afs/cern.ch/sw/XML/TL2007/texmf-dist/tex/latex/amsfonts/umsb.fd)
Underfull \vbox (badness 2521) detected at line 459
[1{/afs/cern.ch/sw/XML/TL2007/texmf-var/fonts/map/pdftex/updmap/pdftex.map}]
Underfull \vbox (badness 10000) detected at line 459
[2]) [3] (./compass_spec.toc) [4] (./compass_spec_int.tex
Underfull \vbox (badness 10000) has occurred while \output is active
Underfull \vbox (badness 10000) has occurred while \output is active [5])
[6] (./compass_spec_lay.tex
<./figures/Layout-3D-1XL-BW.jpg, id=39, 1828.8325pt x 1008.76875pt>
<use ./figures/Layout-3D-1XL-BW.jpg>
<./figures/compass_setup_2004_bw.pdf, id=40, 1012.78375pt x 532.99126pt>
<use ./figures/compass_setup_2004_bw.pdf>
Underfull \vbox (badness 10000) has occurred while \output is active [7]
[8 <./figures/Layout-3D-1XL-BW.jpg> <./figures/compass_setup_2004_bw.pdf>]
[9] [10] <./figures/Q2_vs_x.pdf, id=65, 569.12625pt x 385.44pt>
<use ./figures/Q2_vs_x.pdf> [11 <./figures/Q2_vs_x.pdf>]) [12]
(./compass_spec_bea.tex [13]
<./figures/m2_muon_polarisation.pdf, id=83, 569.12625pt x 385.44pt>
<use ./figures/m2_muon_polarisation.pdf>
<./figures/m2_muon_flux.jpg, id=84, 569.12625pt x 385.44pt>
<use ./figures/m2_muon_flux.jpg>
Underfull \vbox (badness 10000) has occurred while \output is active [14 <./fig
ures/m2_muon_polarisation.pdf> <./figures/m2_muon_flux.jpg>]
<./figures/bms.pdf, id=104, 762.85pt x 320.19624pt> <use ./figures/bms.pdf>
Underfull \vbox (badness 10000) has occurred while \output is active [15])
[16 <./figures/bms.pdf>] (./compass_spec_tgt.tex
Underfull \vbox (badness 10000) has occurred while \output is active [17]
<./figures/smc-dilu-compass4p.jpg, id=121, 845.1575pt x 597.23125pt>
<use ./figures/smc-dilu-compass4p.jpg>
<./figures/pol04P2ABW.jpg, id=122, 570.13pt x 371.3875pt>
<use ./figures/pol04P2ABW.jpg> [18]) [19 <./figures/smc-dilu-compass4p.jpg>]
[20 <./figures/pol04P2ABW.jpg>] (./compass_spec_trk.tex
(./trk/compass_spec_trk_vsat_scifi.tex
Underfull \vbox (badness 10000) has occurred while \output is active
<./figures/fibrelayout.pdf, id=133, 367.3725pt x 138.5175pt>
<use ./figures/fibrelayout.pdf>
Underfull \vbox (badness 1466) has occurred while \output is active [21 <./figu
res/fibrelayout.pdf>]
<./figures/time_vs_profile_scifi5y.pdf, id=146, 569.12625pt x 385.44pt>
<use ./figures/time_vs_profile_scifi5y.pdf>
Underfull \vbox (badness 10000) has occurred while \output is active)
(./trk/compass_spec_trk_vsat_sil.tex [22 <./figures/time_vs_profile_scifi5y.pdf
>] <./figures/detector-module-4.jpg, id=157, 617.30624pt x 405.515pt>
<use ./figures/detector-module-4.jpg>
<./figures/si_Y_residuum.pdf, id=158, 569.12625pt x 385.44pt>
<use ./figures/si_Y_residuum.pdf>
<./figures/si_X_residuum.pdf, id=159, 569.12625pt x 385.44pt>
<use ./figures/si_X_residuum.pdf>
<./figures/si_time.pdf, id=160, 569.12625pt x 385.44pt>
<use ./figures/si_time.pdf> [23 <./figures/detector-module-4.jpg>])
(./trk/compass_spec_trk_sat_mm.tex
<./figures/mmegas_principle.pdf, id=164, 462.72874pt x 327.2225pt>
<use ./figures/mmegas_principle.pdf> [24 <./figures/si_Y_residuum.pdf> <./figur
es/si_X_residuum.pdf> <./figures/si_time.pdf>]
Overfull \hbox (4.81487pt too wide) in paragraph at lines 42--46
[]\OT1/cmr/m/n/10 The gas mix-ture used is Ne/C$[]$H$[]$/CF$[]$ (80/10/10),
<./figures/mm03_photo_labels.jpg, id=205, 645.00975pt x 487.8225pt>
<use ./figures/mm03_photo_labels.jpg>
<./figures/MM02Y1_TimeRes.pdf, id=206, 569.12625pt x 385.44pt>
<use ./figures/MM02Y1_TimeRes.pdf> [25 <./figures/mmegas_principle.pdf> <./figu
res/mm03_photo_labels.jpg>]
<./figures/MM02Y1_SpatRes.pdf, id=214, 569.12625pt x 385.44pt>
<use ./figures/MM02Y1_SpatRes.pdf>) (./trk/compass_spec_trk_sat_gem.tex
<./figures/TGEM_principle_field.jpg, id=215, 149.52414pt x 86.4748pt>
<use ./figures/TGEM_principle_field.jpg> [26 <./figures/MM02Y1_TimeRes.pdf> <./
figures/MM02Y1_SpatRes.pdf> <./figures/TGEM_principle_field.jpg>]
<./figures/2d-PCB_v2.jpg, id=242, 235.23885pt x 160.4394pt>
<use ./figures/2d-PCB_v2.jpg>
<./figures/GM02X_SpatialResolution_GEMTracking_22019_StrdOpt_grey_v2.pdf, id=24
3, 569.12625pt x 385.44pt>
<use ./figures/GM02X_SpatialResolution_GEMTracking_22019_StrdOpt_grey_v2.pdf>
[27 <./figures/2d-PCB_v2.jpg>]
<./figures/GM06U_TimeResolution_22019_grey_v3.pdf, id=247, 569.12625pt x 385.44
pt> <use ./figures/GM06U_TimeResolution_22019_grey_v3.pdf>)
(./trk/compass_spec_trk_lat_dc.tex [28 <./figures/GM02X_SpatialResolution_GEMTr
acking_22019_StrdOpt_grey_v2.pdf> <./figures/GM06U_TimeResolution_22019_grey_v3
.pdf>] <./figures/trk_dc_cell.pdf, id=273, 149.55875pt x 99.37125pt>
<use ./figures/trk_dc_cell.pdf>
<./figures/DC01U1_rates.pdf, id=274, 569.12625pt x 385.44pt>
<use ./figures/DC01U1_rates.pdf>
<./figures/DC01X_RT.jpg, id=275, 569.12625pt x 385.44pt>
<use ./figures/DC01X_RT.jpg> [29 <./figures/trk_dc_cell.pdf> <./figures/DC01U1_
rates.pdf>] <./figures/DC01X1_resolution.pdf, id=316, 569.12625pt x 385.44pt>
<use ./figures/DC01X1_resolution.pdf>) (./trk/compass_spec_trk_lat_straw.tex
<figures/straw_fig1_v2.pdf, id=317, 578.16pt x 352.31625pt>
<use figures/straw_fig1_v2.pdf> [30 <./figures/DC01X_RT.jpg> <./figures/DC01X1_
resolution.pdf> <./figures/straw_fig1_v2.pdf>]
Underfull \hbox (badness 10000) in paragraph at lines 81--81
[][]

Underfull \hbox (badness 10000) in paragraph at lines 81--82
[]\OT1/cmr/m/n/8 Length

Underfull \hbox (badness 10000) in paragraph at lines 81--82
[]

Underfull \hbox (badness 10000) in paragraph at lines 83--83
[]\OT1/cmr/m/n/8 Number

Underfull \hbox (badness 10000) in paragraph at lines 83--83
[]

Underfull \vbox (badness 10000) has occurred while \output is active
<figures/ST03U1db_RT.pdf, id=340, 569.12625pt x 385.44pt>
<use figures/ST03U1db_RT.pdf>
<figures/ST03X1db_residual_vs_ch.pdf, id=341, 569.12625pt x 385.44pt>
<use figures/ST03X1db_residual_vs_ch.pdf> [31 <./figures/ST03U1db_RT.pdf>])
(./trk/compass_spec_trk_lat_mwpc.tex
Underfull \vbox (badness 10000) has occurred while \output is active [32 <./fig
ures/ST03X1db_residual_vs_ch.pdf>]
<figures/tracking_mwpc_residuals.pdf, id=376, 569.12625pt x 385.44pt>
<use figures/tracking_mwpc_residuals.pdf>
<figures/tracking_mwpc_residuals_cls12.pdf, id=377, 569.12625pt x 385.44pt>
<use figures/tracking_mwpc_residuals_cls12.pdf>
Underfull \vbox (badness 10000) has occurred while \output is active
<figures/tracking_mwpc_efficiency.pdf, id=378, 569.12625pt x 385.44pt>
<use figures/tracking_mwpc_efficiency.pdf> [33 <./figures/tracking_mwpc_residua
ls.pdf> <./figures/tracking_mwpc_residuals_cls12.pdf>])
(./trk/compass_spec_trk_lat_w45.tex
<figures/W45_wire_thick.jpg, id=409, 1606.0pt x 1204.5pt>
<use figures/W45_wire_thick.jpg>
<figures/W45_RT.pdf, id=410, 569.12625pt x 385.44pt> <use figures/W45_RT.pdf>))
 [34 <./figures/tracking_mwpc_efficiency.pdf> <./figures/W45_wire_thick.jpg> <.
/figures/W45_RT.pdf>] [35] (./compass_spec_pid.tex
(./pid/compass_spec_pid_lat_rich.tex
<./figures/pid/rich/principle.jpg, id=431, 910.40125pt x 483.8075pt>
<use ./figures/pid/rich/principle.jpg>
Underfull \vbox (badness 3503) has occurred while \output is active [36]
<./figures/pid/rich/gas_transparency.pdf, id=435, 569.12625pt x 385.44pt>
<use ./figures/pid/rich/gas_transparency.pdf> [37 <./figures/pid/rich/principle
.jpg> <./figures/pid/rich/gas_transparency.pdf>]
<./figures/pid/rich/mirror_reflectance.pdf, id=456, 569.12625pt x 385.44pt>
<use ./figures/pid/rich/mirror_reflectance.pdf>
Underfull \hbox (badness 3861) in paragraph at lines 191--205
\OT1/cmr/m/n/10 1 is equipped with eight large-size MW-PCs
<./figures/pid/rich/RICH-detector.pdf, id=457, 378.50711pt x 193.33731pt>
<use ./figures/pid/rich/RICH-detector.pdf> [38 <./figures/pid/rich/mirror_refle
ctance.pdf> <./figures/pid/rich/RICH-detector.pdf>]
<./figures/pid/rich/ro_scheme.jpg, id=489, 594.22pt x 843.15pt>
<use ./figures/pid/rich/ro_scheme.jpg>
<./figures/pid/rich/event-display.jpg, id=490, 370.0224pt x 412.6617pt>
<use ./figures/pid/rich/event-display.jpg>
Underfull \vbox (badness 3503) has occurred while \output is active
<./figures/pid/rich/Nphotons.jpg, id=491, 511.9125pt x 255.95625pt>
<use ./figures/pid/rich/Nphotons.jpg>
<./figures/pid/rich/PhotonResolution.jpg, id=492, 460.72125pt x 233.87375pt>
<use ./figures/pid/rich/PhotonResolution.jpg>
<./figures/pid/rich/RingResolution.jpg, id=493, 547.04375pt x 391.4625pt>
<use ./figures/pid/rich/RingResolution.jpg>
Underfull \vbox (badness 3503) has occurred while \output is active [39])
(./pid/compass_spec_mw.tex
Underfull \vbox (badness 10000) has occurred while \output is active)
(./pid/compass_spec_mw1.tex
Underfull \vbox (badness 10000) has occurred while \output is active [40 <./fig
ures/pid/rich/ro_scheme.jpg>]
<./figures/mw1_mdt.jpg, id=500, 597.6729pt x 845.19765pt>
<use ./figures/mw1_mdt.jpg> [41 <./figures/mw1_mdt.jpg> <./figures/pid/rich/eve
nt-display.jpg> <./figures/pid/rich/Nphotons.jpg> <./figures/pid/rich/PhotonRes
olution.jpg> <./figures/pid/rich/RingResolution.jpg>]
<./figures/mw1_mw1.jpg, id=506, 885.3075pt x 861.2175pt>
<use ./figures/mw1_mw1.jpg>
Underfull \vbox (badness 1769) has occurred while \output is active
<./figures/mw1_eff_2003_2004.pdf, id=508, 569.12625pt x 385.44pt>
<use ./figures/mw1_eff_2003_2004.pdf>) (./pid/compass_spec_pid_lat_mw2.tex
<./figures/MW2_tub_lay.pdf, id=509, 463.7325pt x 291.0875pt>
<use ./figures/MW2_tub_lay.pdf>
Underfull \vbox (badness 3503) has occurred while \output is active [42 <./figu
res/mw1_mw1.jpg>]
Underfull \vbox (badness 10000) has occurred while \output is active [43 <./fig
ures/MW2_tub_lay.pdf> <./figures/mw1_eff_2003_2004.pdf>]
<./figures/tracking_mw2.jpg, id=540, 569.12625pt x 385.44pt>
<use ./figures/tracking_mw2.jpg>
Underfull \vbox (badness 1603) has occurred while \output is active)
(./pid/compass_spec_pid_calo.tex) (./hcal1/compass_spec_calo_hcal_hcal1.tex
<figures/hcal1_module.pdf, id=541, 542.025pt x 342.27875pt>
<use figures/hcal1_module.pdf>
Underfull \hbox (badness 5417) in paragraph at lines 40--58
\OT1/cmr/m/n/10 terphenyl ($1\OML/cmm/m/it/10 :\OT1/cmr/m/n/10 5 %$) and POPOP 
(1,4-Bis-[2-(5-
[44 <./figures/tracking_mw2.jpg>]
<figures/HCAL1_E_vs_p.pdf, id=545, 569.12625pt x 552.0625pt>
<use figures/HCAL1_E_vs_p.pdf>
<figures/HCAL1_reso.pdf, id=547, 569.12625pt x 552.0625pt>
<use figures/HCAL1_reso.pdf>) (./pid/compass_spec_pid_hcal2.tex
Underfull \vbox (badness 3503) has occurred while \output is active [45 <./figu
res/hcal1_module.pdf>]
<./figures/hcal2_fibre.pdf, id=555, 614.295pt x 794.97pt>
<use ./figures/hcal2_fibre.pdf>
<./figures/hcal2_energy_resolution.pdf, id=556, 421.575pt x 298.11375pt>
<use ./figures/hcal2_energy_resolution.pdf> [46 <./figures/HCAL1_E_vs_p.pdf> <.
/figures/HCAL1_reso.pdf> <./figures/hcal2_fibre.pdf>])
(./pid/compass_spec_pid_calo_ecal.tex
<./figures/LG_blocks_new.pdf, id=600, 597.23125pt x 845.1575pt>
<use ./figures/LG_blocks_new.pdf>))
Underfull \vbox (badness 1215) has occurred while \output is active [47 <./figu
res/LG_blocks_new.pdf> <./figures/hcal2_energy_resolution.pdf>] [48]
(./compass_spec_trg.tex (./trg/compass_spec_trg_muon.tex
<./figures/trigger_concept4_paper.pdf, id=620, 524.96124pt x 501.875pt>
<use ./figures/trigger_concept4_paper.pdf>
<./figures/setup_2001.pdf, id=621, 1926.19624pt x 912.40875pt>
<use ./figures/setup_2001.pdf> [49 <./figures/trigger_concept4_paper.pdf> <./fi
gures/setup_2001.pdf>]
Underfull \vbox (badness 3503) has occurred while \output is active [50]
<./figures/veto2d.pdf, id=664, 569.12625pt x 327.2225pt>
<use ./figures/veto2d.pdf>
<./figures/qq2y_160.pdf, id=665, 569.12625pt x 546.04pt>
<use ./figures/qq2y_160.pdf>) (./trg/compass_spec_trg_hadron.tex [51 <./figures
/veto2d.pdf>]
<figures/primakoff_trigger.pdf, id=680, 669.50125pt x 181.67876pt>
<use figures/primakoff_trigger.pdf>
Underfull \vbox (badness 10000) has occurred while \output is active [52 <./fig
ures/qq2y_160.pdf>])) [53 <./figures/primakoff_trigger.pdf>]
(./compass_spec_daq.tex (./daq/compass_spec_daq_overview.tex
<./figures/daq-overview.pdf, id=707, 460.72125pt x 405.515pt>
<use ./figures/daq-overview.pdf>
Underfull \vbox (badness 10000) has occurred while \output is active [54 <./fig
ures/daq-overview.pdf>]) (./daq/compass_spec_daq_tcs.tex
<./figures/tcs.pdf, id=724, 274.02374pt x 416.55624pt> <use ./figures/tcs.pdf>
[55 <./figures/tcs.pdf>]) (./daq/compass_spec_daq_digitisation.tex)
(./daq/compass_spec_daq_sgadc.tex) (./daq/compass_spec_daq_caladc.tex
Underfull \vbox (badness 3503) has occurred while \output is active [56])
(./daq/compass_spec_daq_f1tdc.tex
Underfull \vbox (badness 3503) has occurred while \output is active [57])
(./daq/compass_spec_daq_catch.tex
<./figures/daq-catch.pdf, id=743, 886.31125pt x 516.93124pt>
<use ./figures/daq-catch.pdf> [58 <./figures/daq-catch.pdf>]
<figures/mwpc_readout.pdf, id=756, 931.48pt x 617.30624pt>
<use figures/mwpc_readout.pdf>
Underfull \vbox (badness 3503) has occurred while \output is active)
(./daq/compass_spec_daq_gesica.tex [59]
Underfull \vbox (badness 10000) has occurred while \output is active
Underfull \vbox (badness 10000) has occurred while \output is active [60 <./fig
ures/mwpc_readout.pdf>]) (./daq/compass_spec_daq_daq.tex
Underfull \vbox (badness 3503) has occurred while \output is active [61]
Underfull \vbox (badness 3503) has occurred while \output is active
Underfull \vbox (badness 3503) has occurred while \output is active [62]))
[63] (./compass_spec_onl.tex [64]
<./figures/DCS.jpg, id=782, 532.99126pt x 237.88875pt> <use ./figures/DCS.jpg>
[65]) [66 <./figures/DCS.jpg>] (./compass_spec_per.tex
<./figures/reco_flow_chart.pdf, id=789, 1028.84375pt x 1910.13625pt>
<use ./figures/reco_flow_chart.pdf>
Underfull \vbox (badness 10000) has occurred while \output is active [67 <./fig
ures/reco_flow_chart.pdf>] [68]
Underfull \vbox (badness 10000) has occurred while \output is active
Underfull \vbox (badness 10000) has occurred while \output is active [69]
<./figures/vert_profile.pdf, id=804, 569.12625pt x 355.3275pt>
<use ./figures/vert_profile.pdf>
<./figures/vert_sigmaZ_vs_z.jpg, id=805, 569.12625pt x 369.38pt>
<use ./figures/vert_sigmaZ_vs_z.jpg>
<figures/kaon_mass.pdf, id=806, 539.01375pt x 390.45876pt>
<use figures/kaon_mass.pdf>
<figures/lambda_mass.pdf, id=808, 541.02126pt x 390.45876pt>
<use figures/lambda_mass.pdf> [70 <./figures/kaon_mass.pdf> <./figures/lambda_m
ass.pdf> <./figures/vert_profile.pdf> <./figures/vert_sigmaZ_vs_z.jpg>]
[71] <figures/tracking_acceptance.pdf, id=850, 569.12625pt x 385.44pt>
<use figures/tracking_acceptance.pdf>
<figures/tracking_efficiency.pdf, id=852, 569.12625pt x 385.44pt>
<use figures/tracking_efficiency.pdf>
<figures/resolMag.pdf, id=854, 569.12625pt x 387.4475pt>
<use figures/resolMag.pdf>
<figures/Offline_ResolTheta.pdf, id=856, 570.13pt x 394.47375pt>
<use figures/Offline_ResolTheta.pdf>
<./figures/pid/rich/cherenkov_angle_vs_momentum.jpg, id=858, 718.685pt x 693.59
125pt> <use ./figures/pid/rich/cherenkov_angle_vs_momentum.jpg>
<./figures/pid/rich/rich_efficiency_1.pdf, id=859, 569.12625pt x 541.02126pt>
<use ./figures/pid/rich/rich_efficiency_1.pdf>
<./figures/pid/rich/rich_efficiency_2.pdf, id=860, 569.12625pt x 541.02126pt>
<use ./figures/pid/rich/rich_efficiency_2.pdf> [72 <./figures/tracking_acceptan
ce.pdf> <./figures/tracking_efficiency.pdf>]
<./figures/pid/rich/purity.jpg, id=900, 511.9125pt x 541.02126pt>
<use ./figures/pid/rich/purity.jpg>
Underfull \vbox (badness 10000) has occurred while \output is active [73 <./fig
ures/resolMag.pdf> <./figures/Offline_ResolTheta.pdf> <./figures/pid/rich/chere
nkov_angle_vs_momentum.jpg>]
Underfull \vbox (badness 1210) has occurred while \output is active
Underfull \vbox (badness 10000) has occurred while \output is active [74 <./fig
ures/pid/rich/rich_efficiency_1.pdf> <./figures/pid/rich/rich_efficiency_2.pdf>
 <./figures/pid/rich/purity.jpg>]
<./figures/eta_mass.pdf, id=964, 569.12625pt x 365.365pt>
<use ./figures/eta_mass.pdf>) [75 <./figures/eta_mass.pdf>]
(./compass_spec_upg.tex [76] [77]
Underfull \vbox (badness 3503) has occurred while \output is active [78])
[79] (./compass_spec_sum.tex
Underfull \hbox (badness 7415) in paragraph at lines 3--33
\OT1/cmr/m/n/10 calorime-ter in-for-ma-tion. Sev-eral custom-made

Underfull \vbox (badness 10000) has occurred while \output is active) [80]
(./compass_spec_ack.tex) [81] (./compass_spec.bbl
Underfull \hbox (badness 7944) in paragraph at lines 72--75
[]\OT1/cmr/m/n/8 A. Meier, $[]$LiD f^^?ur das Po-lar-isierte Tar-get

Underfull \hbox (badness 10000) in paragraph at lines 118--120
[]\OT1/cmr/m/n/8 Hamamatsu Pho-ton-ics K.K., 14-

Underfull \hbox (badness 10000) in paragraph at lines 152--153
[]\OT1/cmr/m/n/8 Kaneka Cor-po-ra-tion, Pasadena, USA,
[82]
Underfull \hbox (badness 10000) in paragraph at lines 219--220
[]\OT1/cmr/m/n/8 RD26 Col-lab-o-ra-tion, RD26 sta-tus re-port,

Underfull \hbox (badness 10000) in paragraph at lines 222--223
[]\OT1/cmr/m/n/8 RD26 Col-lab-o-ra-tion, RD26 sta-tus re-port,

Underfull \hbox (badness 10000) in paragraph at lines 225--226
[]\OT1/cmr/m/n/8 RD26 Col-lab-o-ra-tion, RD26 sta-tus re-port,

Underfull \hbox (badness 10000) in paragraph at lines 315--317
\OT1/cmr/m/n/8 Com-put-ing in high en-ergy and

Underfull \hbox (badness 6157) in paragraph at lines 325--327
[]\OT1/cmr/m/n/8 iseg Spezialelek-tronik GmbH, 01454 Rade-berg,

Underfull \hbox (badness 10000) in paragraph at lines 339--340
[]\OT1/cmr/m/n/8 The OPC Foun-da-tion,

Underfull \hbox (badness 10000) in paragraph at lines 348--352
[]\OT1/cmr/m/n/8 D. R. My-ers, et al., The

Underfull \hbox (badness 10000) in paragraph at lines 348--352
\OT1/cmr/m/n/8 http://accelconf.web.cern.ch/AccelConf/ica99

Underfull \hbox (badness 10000) in paragraph at lines 354--355
[][] \OT1/cmr/m/n/8 AB, 753 20 Up-p-sala, Swe-den,

Underfull \hbox (badness 10000) in paragraph at lines 381--384
\OT1/cmr/m/n/8 http://wwwasdoc.web.cern.ch/wwwasdoc
[83]) [84] (./compass_spec.aux (./compass_spec_tit.aux) (./compass_spec_int.aux
) (./compass_spec_lay.aux) (./compass_spec_bea.aux) (./compass_spec_tgt.aux)
(./compass_spec_trk.aux) (./compass_spec_pid.aux) (./compass_spec_trg.aux)
(./compass_spec_daq.aux) (./compass_spec_onl.aux) (./compass_spec_per.aux)
(./compass_spec_upg.aux) (./compass_spec_sum.aux) (./compass_spec_ack.aux)) )
(see the transcript file for additional information)</afs/cern.ch/sw/XML/TL2007
/texmf-dist/fonts/type1/bluesky/cm/cmbx10.pfb></afs/cern.ch/sw/XML/TL2007/texmf
-dist/fonts/type1/bluesky/cm/cmbx8.pfb></afs/cern.ch/sw/XML/TL2007/texmf-dist/f
onts/type1/bluesky/cm/cmbx9.pfb></afs/cern.ch/sw/XML/TL2007/texmf-dist/fonts/ty
pe1/bluesky/cm/cmcsc10.pfb></afs/cern.ch/sw/XML/TL2007/texmf-dist/fonts/type1/b
luesky/cm/cmex10.pfb></afs/cern.ch/sw/XML/TL2007/texmf-dist/fonts/type1/bluesky
/cm/cmmi10.pfb></afs/cern.ch/sw/XML/TL2007/texmf-dist/fonts/type1/bluesky/cm/cm
mi6.pfb></afs/cern.ch/sw/XML/TL2007/texmf-dist/fonts/type1/bluesky/cm/cmmi7.pfb
></afs/cern.ch/sw/XML/TL2007/texmf-dist/fonts/type1/bluesky/cm/cmmi8.pfb></afs/
cern.ch/sw/XML/TL2007/texmf-dist/fonts/type1/bluesky/cm/cmr10.pfb></afs/cern.ch
/sw/XML/TL2007/texmf-dist/fonts/type1/bluesky/cm/cmr12.pfb></afs/cern.ch/sw/XML
/TL2007/texmf-dist/fonts/type1/bluesky/cm/cmr17.pfb></afs/cern.ch/sw/XML/TL2007
/texmf-dist/fonts/type1/bluesky/cm/cmr6.pfb></afs/cern.ch/sw/XML/TL2007/texmf-d
ist/fonts/type1/bluesky/cm/cmr7.pfb></afs/cern.ch/sw/XML/TL2007/texmf-dist/font
s/type1/bluesky/cm/cmr8.pfb></afs/cern.ch/sw/XML/TL2007/texmf-dist/fonts/type1/
bluesky/cm/cmr9.pfb></afs/cern.ch/sw/XML/TL2007/texmf-dist/fonts/type1/bluesky/
cm/cmsl8.pfb></afs/cern.ch/sw/XML/TL2007/texmf-dist/fonts/type1/bluesky/cm/cmsy
10.pfb></afs/cern.ch/sw/XML/TL2007/texmf-dist/fonts/type1/bluesky/cm/cmsy6.pfb>
</afs/cern.ch/sw/XML/TL2007/texmf-dist/fonts/type1/bluesky/cm/cmsy7.pfb></afs/c
ern.ch/sw/XML/TL2007/texmf-dist/fonts/type1/bluesky/cm/cmsy8.pfb></afs/cern.ch/
sw/XML/TL2007/texmf-dist/fonts/type1/bluesky/cm/cmti10.pfb></afs/cern.ch/sw/XML
/TL2007/texmf-dist/fonts/type1/bluesky/cm/cmti8.pfb></afs/cern.ch/sw/XML/TL2007
/texmf-dist/fonts/type1/bluesky/ams/msam10.pfb></afs/cern.ch/sw/XML/TL2007/texm
f-local/fonts/type1/public/pscyr/times.pfb>
Output written on compass_spec.pdf (84 pages, 2292645 bytes).
Transcript written on compass_spec.log.

